Robust Distillation for Worst-class Performance

Knowledge distillation has proven to be an effective technique in improving the performance a student model using predictions from a teacher model. However, recent work has shown that gains in average efficiency are not uniform across subgroups in the data, and in particular can often come at the cost of accuracy on rare subgroups and classes. To preserve strong performance across classes that may follow a long-tailed distribution, we develop distillation techniques that are tailored to improve the student's worst-class performance. Specifically, we introduce robust optimization objectives in different combinations for the teacher and student, and further allow for training with any tradeoff between the overall accuracy and the robust worst-class objective. We show empirically that our robust distillation techniques not only achieve better worst-class performance, but also lead to Pareto improvement in the tradeoff between overall performance and worst-class performance compared to other baseline methods. Theoretically, we provide insights into what makes a good teacher when the goal is to train a robust student.

==> robust-distillation (1)/algorithms.tex <==
\section{Robust Distillation Algorithms}
\label{sec:algorithms}
The different objectives we consider -- standard, balanced and robust -- entail different loss objectives to ensure efficient optimization during training.
% Having outlined our main distillation proposal, 
% we now describe the algorithms we use to optimize the different teacher and student objectives.
% During the training phase, however, we employ differentiable surrogates for efficient optimization.
For example, while training
the standard teacher and student in \eqref{eq:standard-objectives},
we take $\ell$ to be the softmax cross-entropy loss,
and optimize it using SGD. For the balanced and robust models,
we employ the margin-based surrogates that we detail below, which have shown to be more effective
in training over-parameterized networks \citep{cao2019learning, menon2020long, kini2021labelimbalanced}. 
Across all objectives, at evaluation we take the loss $\ell$ 
in the student and teacher objectives
to be the 0-1 loss. 



\textbf{Margin-based surrogate for balanced objective.}\
When the teacher or student model being trained is over-parameterized,
i.e., has sufficient capacity to correctly classify all examples in the training set,
the use of an outer weighting term 
in the objective
(such as the inverse class marginals in \eqref{eq:balanced-distilled-empirical})
can be ineffective. In other words, a model that yields zero training objective
would do so irrespective of what outer weights we choose. 
To remedy this problem,
we make use of the margin-based surrogate of \citet{menon2020long},
and incorporate the outer weights as margin terms within the loss. 
For
the balanced student objective in \eqref{eq:balanced-distilled-empirical}, this would look like:
\begin{align}
    {\widetilde{L}^\bald(f^s)}
    &= \frac{1}{n}\sum_{i=1}^n \cL^\mar\left(p^t(x_i), f^s(x_i); \1 / \hat{\pi}^t \right),
    \label{eq:margin-la}
\end{align}
~\\[-25pt]
%where $\hat{\pi}_y^t = \frac{1}{\frac{1}{n}\sum_{i=1}^n p^t_y(x_i)}$, and
\begin{align}
\text{where}~~\cL^\mar\left(\bp, \boldf; \bc \right) &=
\frac{1}{m}\sum_{y \in [m]} p_y \log\bigg(1 + \sum_{j \ne y}\exp\left(\log(c_y / c_{j}) \,-\, (f_y - f_j) \right) \bigg),
\nonumber
\end{align}
for teacher probabilities $\bp \in \Delta_m$, student scores $\boldf \in \R^m$,
and per-class costs $\bc \in \R^m_+$. 
 For the balanced teacher, the margin-based objective would take a similar form, but %would instead
 with one-hot labels. 


We include a proof in Appendix \ref{app:calibration-mar} showing that
a scoring function that minimizes this surrogate objective
also minimizes the
the balanced objective in \eqref{eq:balanced-distilled-empirical}
(when $\ell$ is the cross-entropy loss, and the student is chosen from a sufficiently flexible function class). In practice, the margin term $\log(c_y / c_{j})$ encourages a larger margin of separation for classes $y$ for which the cost $c_y$ is relatively higher.
 
\begin{figure}[t]
\vspace{-5pt}
\begin{algorithm}[H]
\caption{Distilled Margin-based DRO}% for Robust Student}
\label{algo:dro}
\begin{algorithmic}
\STATE \textbf{Inputs:} Teacher $p^t$, Student hypothesis class $\cF$, Training set $S$, Validation set $S^\val$, Step-size $\gamma \in \R_+$,
Number of iterations $K$, Loss $\ell$,
Initial student $f^0 \in \cF$, Initial multipliers $\blambda^0 \in \Delta_m$
\STATE Compute $\hat{\pi}^{t}_j = \frac{1}{n}\sum_{(x, y) \in S} p_j^t(x),~ \forall j \in [m]$
\STATE Compute $\hat{\pi}^{t,\val}_j = \frac{1}{n^\val}\sum_{(x, y) \in S^\val} p_j^t(x),~ \forall j \in [m]$
\STATE \textbf{For}~{$k = 0 $ to $K-1$}
\STATE ~~~$\tilde{\lambda}^{k+1}_j \,=\, \lambda^k_j\exp\big( \gamma \hat{R}_j \big), \forall j \in [m]$%\todo{[Hari] Change step size in appendix to $\gamma$}
~~~~~\text{where} $\hat{R}_j =$ $\frac{1}{n^\val}\frac{1}{\hat{\pi}^{t,\val}_j}\underset{(x, y) \in S^\val}{\sum} p_j^t(x)\, \ell( j , f^k(x) )$\\[-20pt]
% \STATE ~~~~~~~~~$\begin{cases} 
%             \displaystyle\frac{1}{|S^\val|}\frac{1}{\hat{\pi}^t_j}\sum_{(x, y) \in S^\val} p_j^t(x_i)\, \ell( j , f^k(x) ) & \text{:A}\\
%             \displaystyle\frac{1}{|S^\val|}\frac{1}{\hat{\pi}_j}\sum_{(x, y) \in S^\val} \1(y=j)\,\ell( j , f^k(x) ) & \text{:B}
%         \end{cases}$
%\frac{1}{n^\val\hat{\pi}^t_y}\sum_{ p_y^t(x_i)\, \ell\left( y , f^k(x_i) \right)
\STATE ~~~$\lambda^{k+1}_y \,=\, \frac{\tilde{\lambda}^{k+1}_y}{\sum_{j=1}^m \tilde{\lambda}^{k+1}_j}, \forall y$
\STATE ~~~$f^{k+1} \,\in\, \Argmin{f \in \cF}\, \frac{1}{n}\sum_{i=1}^n \cL^\mar\left(p^t(x_i), f(x_i); \frac{\lambda^{k+1}}{\hat{\pi}^t} \right)$
~~~~~~// Replaced with a few steps of SGD
\STATE \textbf{End For}
\STATE \textbf{Output:} $\bar{f}^{s}: x \mapsto \frac{1}{K}\sum_{k =1}^K f^k(x)$
\end{algorithmic}
\end{algorithm}
\vspace{-22pt}
\end{figure} 
 
 
\textbf{Margin-based DRO for robust objective.}\
% For the robust teacher, we the 
% procedure
% proposed by \citet{narasimhan2021training}, 
% which we refer to as worst-class distributionally-robust optimization (DRO).
% For the robust student, we consider two variants of this procedure, we elaborate next.
Minimizing the robust objective with plain SGD can be difficult due to the presence of
the outer ``max'' over $m$ classes. The key difficulty is in computing reliable stochastic gradients for
the max objective, especially given a small batch size. The
standard approach is to instead use a (group) distributionally-robust optimization (DRO) procedure,
which comes in multiple flavors \cite{chen2017robust, Sagawa2020Distributionally, kini2021labelimbalanced}.
We employ  the margin-based variant of group DRO  \citep{narasimhan2021training} as it naturally extends the 
margin-based objective used in the balanced setting.

We illustrate below how this applies to the robust student objective in \eqref{eq:robust-distilled-empirical}. The procedure for the robust teacher is similar, but involves one-hot labels.
For a student hypothesis class $\cF$,
%Parameterizing student $f$ with $\theta \in \R^d$,
we
first re-write the minimization in \eqref{eq:robust-distilled-empirical} 
over $f \in \cF$ into an equivalent min-max optimization using per-class multipliers $\lambda \in \Delta_m$:
\vspace{-5pt}
\[
\min_{f \in \cF}\max_{\lambda \in \Delta_m} \sum_{y \in [m]}\frac{\lambda_y}{\hat{\pi}^t_y}\frac{1}{n}\sum_{i=1}^n  p_y^t(x_i)\, \ell\left( y , f(x_i) \right),
\]
and then
 maximize over $\lambda$ for fixed $f$, and minimize over $f$ for fixed $\lambda$:
%  $\lambda^{k+1}_y \propto 
%     \lambda^k_y\exp\bigg( \gamma\frac{1}{n\hat{\pi}^t_y}\sum_{i=1}^n  p_y^t(x_i) \ell\left( y , f^k(x_i) \right)\bigg)$; \\ $f^{k+1} \in \Argmin{f \in \cF} \sum_{y \in [m]}\frac{\lambda^{k+1}_y}{n\hat{\pi}^t_y}\sum_{i=1}^n  p_y^t(x_i) \ell\left( y , f(x_i) \right)$,
\begin{align*}
    \lambda^{k+1}_y &\propto\, 
    \lambda^k_y\exp\bigg( \gamma\frac{1}{n\hat{\pi}^t_y}\sum_{i=1}^n  p_y^t(x_i)\, \ell\left( y , f^k(x_i) \right) \bigg), \forall y\\[-4pt]
    f^{k+1} &\in\, \Argmin{f \in \cF} \sum_{y \in [m]}\frac{\lambda^{k+1}_y}{n\hat{\pi}^t_y}\sum_{i=1}^n  p_y^t(x_i)\, \ell\left( y , f(x_i) \right),
\end{align*}
%
where $\gamma > 0$ is a step-size parameter. The updates on $\lambda$ 
implement exponentiated gradient (EG) ascent to maximize over the simplex \citep{shalev2011online}.

Following \citet{narasimhan2021training}, we make two modifications to the above updates 
when used to train over-parameterized networks that can fit the training set perfectly.
First, we perform the updates on $\lambda$ using a
small held-out validation set $S^\val \,=\, \{(x_1,y_1), \ldots, (x_{n^\val}, y_{n^\val})\}$, 
instead of the training set,
so that the $\lambda$s reflect how well the model generalizes out-of-sample.
Second, in keeping with the balanced objective, we modify the weighted objective
in the $f$-minimization step to include a margin-based surrogate. 
Algorithm \ref{algo:dro}
provides a summary of these steps
and returns a scorer
that averages over the $K$ iterates: $\bar{f}^s(x) = \frac{1}{K}\sum_{k=1}^K f^k(x)$.
While the averaging is needed for our theoretical analysis,
in practice, we find it sufficient to return the last scorer $f^{K}$. 
In Appendix \ref{app:dro-general-algo},
we describe how Algorithm \ref{algo:dro-general} can be easily modified to  trade-off
between the balanced and robust objectives, as shown in \eqref{eq:trade-off-distilled}.

\textbf{To distill the validation set or not?}\
The updates on $\lambda$
in Algorithm \ref{algo:dro} use a validation set labeled by the teacher. 
One could instead perform these updates with a curated validation set containing the original one-hot labels.
 Each of these choices presents different merits. The use of a teacher-labeled validation set is useful
 in many real world scenarios where labeled data is hard to obtain, % \citep{Khan2021,dixon2017,veale_2017}, 
 while unlabeled data abounds.
  In contrast, the use of one-hot validation labels, although more expensive to obtain,  may
make the student more immune to errors in the teacher's predictions, 
as the coefficients $\lambda$s are now based on an unbiased estimate of 
the student's performance on each class.
%
% The use of a validation set for updates on $\lambda$ brings up an interesting
% question: 
% \textit{Would the student be better-off having the validation set also labeled by the teacher?}
% This would be advantageous in many real world scenarios where labeled data is hard to obtain \citep{Khan2021,dixon2017,veale_2017}, while unlabeled data abounds.
% We compare this variant to performance given a curated validation set with the original one-hot labels. While more expensive to obtain a curated validation set, the use of one-hot validation labels may
% %enjoy the best of both worlds: it would benefit from the teacher's 
% % confidence  scores on the training examples, and also be able to make use of the one-hot labels 
% % in the validation set to get an unbiased estimate of its performance on each class. This way, the student
% make the student more immune to errors in the teacher's predictions, 
% as the coefficients $\lambda$s are now based on an unbiased estimate of 
% the student's performance on each class.
%
%  or retaining the original one-hot labels in the validation set, if available?
%  We will experiment with both these versions of DRO, andfor the latter
%
With a one-hot validation set, we update $\lambda$s as follows: %when using a one-hot validation set:
\begin{equation}
    \lambda^{k+1}_j \,=\, \lambda^k_j\exp\big( \eta \hat{R}_j \big), \forall j \in [m], 
~~~~\text{where}~
\hat{R}_j = \frac{1}{n^\val}\frac{1}{\hat{\pi}_j}\sum_{(x, y) \in S^\val} \1(y=j)\,\ell( j , f^k(x) ),
\label{eq:one-hot-val}
\end{equation}
for estimates $\hat{\pi}_y \approx \pi_y$ of the original class priors.
% : (A) we
% can either use
% the teacher's predictions $p^t(x)$ to label the validation set, and (B) or retain
% the original one-hot labels in the validation set (along with estimates of the
% original class priors $\hat{\pi}_y \approx \pi_y$ for the normalizations). 
%
We analyze both the variants in our experiments, and in the next section, discuss robustness guarantees for each.
% Interestingly, \citet{narasimhan2021training} also work with one-hot validation labels
% in their distillation experiments, but do not provide a reasoning for their choice. 
%We revisit the use of
%  one-hot validation labels in the next section. %, and attempt to provide a theoretical justification for it.


%We point the readers to the prior literature on min-max robust optimization \cite{cotter2019optimization, cotter2019training, narasimhan2021training} for 
% In Appendix \ref{app:convergence-dro}, 
% %we extend prior results \cite{cotter2019optimization, cotter2019training, narasimhan2021training} to
% we show that
%  both variants of Algorithm \ref{algo:dro} converge (in the large sample limit) to an optimal solution for \eqref{eq:robust-distilled-empirical}, with variant (B) requiring a milder assumption on the teacher model.
%  \todo{[Hari] Provide formal convergence guarantee for both (A) and (B)}
% We also note that while the algorithm prescribes an exact optimization over $f \in \cF$,
% in practice, we find it sufficient to perform this approximately with a few steps of SGD.
 


% \subsection{Trading-off balanced and worst-class objectives}
% \todo{[Hari] Move to Sec \ref{sec:theory}}
% It is often seen in prior works that training a model
% to achieve good worst-case performance can hurt the model's overall performance \cite{lukasik2021teachers},
% which may not be acceptable in some practical scenarios. Therefore we also consider
% teachers and students that trade-off between the balanced and worst-case performance, e.g., 
% by taking a convex combination
% of the balanced and worst-class objectives:
% \begin{align}
% \text{Teacher:}\hspace{5pt} & \alpha \hat{L}^\bal(f) \,+\, (1 - \alpha)\hat{L}^\rob(f); \nonumber\\
% \text{Student:}\hspace{5pt} & \beta \hat{L}^\bald(f) \,+\, (1 - \beta)\hat{L}^\robd(f),
% \label{eq:trade-off}
% \end{align}
% where $\alpha, \beta \in (0,1)$ are trade-off parameters. 
% Alternatively, one may want to trade-off between the standard and worst-class objectives. 
% A simple variant
% of the group DRO procedure can be applied to solve each of the resulting optimization problems.

==> robust-distillation (1)/distillation.tex <==
\section{Distillation for Worst-class Performance}
\label{sec:distillation}

% Of particular interest to us is the use of 
% knowledge distillation for achieving robust performance.
We adopt the common
practice of training both the teacher and student on the same dataset. Specifically, given a training sample $S = \{(x_1, y_1), \ldots, (x_n, y_n)\}$
drawn from $D$, we first train a teacher model $p^t: \X \> \Delta_m$, and use it to generate a student dataset
$S' = \{(x_1, p^t(x_1)), \ldots, (x_n, p^t(x_n))\}$
by replacing the original labels with the teacher's predictions. %Subsequently, we 
We then train a student scorer $f^s: \X \> [m]$ using the re-labeled dataset,
and use it to construct the final classifier.

% \subsection{Teacher and student objectives}
In a typical setting, both the teacher and student
are trained to optimize a version of the standard objective in \eqref{eq:std}, i.e.,
the teacher is trained to minimize the average loss against the original training labels,
and the student is trained to minimize an average loss against the teacher's predictions:
\begin{align}
        \text{Teacher: } & \hat{L}^\std(f^t) = \frac{1}{n}\sum_{i=1}^n \ell\left( y_i, f^t(x_i) \right); \hspace{10pt}
        \text{Student: } ~ \hat{L}^\stdd(f^s) = \frac{1}{n}\sum_{i=1}^n \sum_{y=1}^m p_y^t(x_i)\, \ell\left(y , f(x_i) \right),\nonumber
    \\[-10pt]\label{eq:standard-objectives}
\end{align}
~\\[-13pt]
% \begin{tabular}{ll}
% Teacher: & 
% \begin{equation}
%     \displaystyle \hat{L}^\std(f^t) = \frac{1}{n}\sum_{i=1}^n \ell\left( y_i, f^t(x_i) \right)\hspace{35pt}
%     \label{eq:standard-objectives}
% \end{equation}
% \\
% Student: & $\displaystyle \hat{L}^\stdd(f^s) = \frac{1}{n}\sum_{i=1}^n \sum_{y=1}^m p_y^t(x_i)\, \ell\left(y , f(x_i) \right),$
% \end{tabular}
% \begin{align}
% \text{Teacher:}\hspace{5pt} \hat{L}^\std(f^t) &= \frac{1}{n}\sum_{i=1}^n \ell\left( y_i, f^t(x_i) \right)
% \label{eq:standard-objectives}
% \\
% \text{Student:}\hspace{5pt} \hat{L}^\stdd(f^s) &= \frac{1}{n}\sum_{i=1}^n \sum_{y=1}^m p_y^t(x_i)\, \ell\left(y , f(x_i) \right),
% \nonumber
% \end{align}
where $p^t(x) = \softmax(f^t(x))$. It is also common to have the student use a mixture of the teacher and one-hot labels. For concreteness, we consider a simpler distillation setup without this mixture, though extensions with this mixture would be straightforward to add.
This work takes a wider view and explores \textit{what combinations of student and teacher objectives} facilitate better worst-group performance for the student. Our experiments evaluate all \emph{nine} combinations of standard, balanced, and robust teacher objectives, paired with standard, balanced, and robust student objectives.

% One option is to change the teacher's objective to either the balanced or robust objectives in \eqref{eq:balanced}--\eqref{eq:robust}, with the goal of yielding better student performance on the tail or more difficult classes. Alternatively, we could alter the student objective to better focus on the more difficult classes.
Given the choice of teacher objective, the student will either optimize a distilled version of the balanced objective in \eqref{eq:balanced}:
\begin{align}
    {\hat{L}^\bald(f^s)}
    &= \frac{1}{m}\sum_{y \in [m]} \frac{1}{\hat{\pi}^t_y}\frac{1}{n}\sum_{i=1}^n  p_y^t(x_i)\, \ell\left( y , f^s(x_i) \right),
    \label{eq:balanced-distilled-empirical}
\end{align}
or a distilled version of the robust objective in \eqref{eq:robust}:
\begin{align}
    {\hat{L}^\robd(f^s)}
    &= \max_{y \in [m]} \frac{1}{\hat{\pi}^t_y}\frac{1}{n}\sum_{i=1}^n  p_y^t(x_i)\, \ell\left( y , f^s(x_i) \right),
    \label{eq:robust-distilled-empirical}
\end{align}
In practice, the teacher's predictions may have a different marginal distribution from the underlying class priors, particularly when temperature scaling is applied to the teacher's logits to soften the predicted probabilities \cite{narasimhan2021training}.  To address this, in both  \eqref{eq:balanced-distilled-empirical} and \eqref{eq:robust-distilled-empirical} we have replaced the class priors $\pi_y$ with the marginal distribution 
 $\hat{\pi}^t_y = \frac{1}{n}\sum_{i=1}^n p^t_y(x_i)$ from the teacher's predictions. 

% balanced
% or robust objectives in \eqref{eq:balanced}--\eqref{eq:robust}, so that
% it yields better performance on the tail or more difficult classes, and in turn 
% enables the student to also perform well on those classes.  Alternatively, 
% we could change the student objective to better focus on the more difficult classes.
% We could either have the student optimize 
% a distilled version of the balanced objective in \eqref{eq:balanced}:
% \begin{align}
%     {\hat{L}^\bald(f^s)}
%     &= \frac{1}{m}\sum_{y \in [m]} \frac{1}{\hat{\pi}^t_y}\frac{1}{n}\sum_{i=1}^n  p_y^t(x_i)\, \ell\left( y , f^s(x_i) \right),
%     \label{eq:balanced-distilled-empirical}
% \end{align}
% or a distilled version of the robust objective in \eqref{eq:robust}:
% \begin{align}
%     {\hat{L}^\robd(f^s)}
%     &= \max_{y \in [m]} \frac{1}{\hat{\pi}^t_y}\frac{1}{n}\sum_{i=1}^n  p_y^t(x_i)\, \ell\left( y , f^s(x_i) \right),
%     \label{eq:robust-distilled-empirical}
% \end{align}
% where we have replaced the class priors $\pi_y$ with the marginal distribution 
%  $\hat{\pi}^t_y = \frac{1}{n}\sum_{i=1}^n p^t_y(x_i)$ from the teacher's predictions. 
% This is because, in practice the teacher's predictions often have a different marginal distribution from the underlying
% class priors, particularly when temperature scaling is applied to the teacher's logits to soften the predicted probabilities \cite{narasimhan2021training}. 

In addition to exploring the combination of objectives that facilitates better worst-group performance for the student, we evaluate a more flexible approach -- have both the teachers and the students trade-off between the balanced and robust objectives:
% resulting in the following optimization objectives:
\begin{align}\label{eq:trade-off-distilled}
        \text{Teacher: } & \hat{L}^\tdf(f^t) = (1-\alpha^t)\hat{L}^\bal(f^t) + \alpha^t\hat{L}^\rob(f^t) \\
        \text{Student: } & \hat{L}^\tdfd(f^s) = (1-\alpha^s)\hat{L}^\bald(f^s) + \alpha^s\hat{L}^\robd(f^s),\nonumber
\end{align}
% \begin{tabular}{ll}
% Teacher: & 
% \hspace{-5pt}
% $
%     \displaystyle\hat{L}^\tdf(f^t) = (1-\alpha^t)\hat{L}^\bal(f^t) + \alpha^t\hat{L}^\rob(f^t)~~~~
%     % \label{eq:trade-off-distilled}
% $ \\
% Student: & $\displaystyle \hat{L}^\tdfd(f^s) = (1-\alpha^s)\hat{L}^\bald(f^s) + \alpha^s\hat{L}^\robd(f^s),$
% \end{tabular}
where $\hat{L}^\bal(f^t)$ and $\hat{L}^\rob(f^t)$ are the respective empirical estimates of
\eqref{eq:balanced} and \eqref{eq:robust} from the training sample, and $\alpha^t, \alpha^s \in [0,1]$
are the respective tradeoff parameters for the teacher and student. %Through these experiments,
We are thus able to evaluate the Pareto-frontier of balanced and worst-case accuracies, obtained from  different combinations of the teachers and students, and 
trained with different trade-off parameters.
%  Of particular interest to us would be the use of the robust objective $\hat{L}^\robd(f)$ for the student,
% which we consider to be the more direct approach. We would first like
% to understand which teachers $p^t$ work well with this objective.




==> robust-distillation (1)/experiments.tex <==
\vspace{-3pt}
\section{Experiments}
\label{sec:expts}
% \vspace{-3pt}
\begin{table*}[t]
\caption{Comparison of \emph{self-distilled} teacher/student combos on test. Worst-class accuracy shown above, standard accuracy shown in parentheses for the top three datasets, and balanced accuracy shown in parenthesis for the bottom two long-tail datasets. Note that $L^{\std} = L^{\bal}$ for the top three datasets with balanced class priors; so here we do not include combinations involving a balanced teacher/student. The combination with the best worst-class accuracy is \textbf{bolded}. Mean and standard error are reported over repeats (10 repeats for CIFAR*, 5 repeats for TinyImageNet). We include results for the robust student using either a teacher labeled validation set (``teacher val''), or true one-hot class labels in the validation set (``one-hot val''), as outlined in Eq.~(\ref{eq:one-hot-val}). We include results using a smaller student architecture (ResNet-56 $\to$ ResNet-32), additional ImageNet results, and additional comparisons to group DRO and the Ada* methods in Appendix \ref{app:experiment_details}.
% \vspace{-10pt}
}
\label{tab:combos}
\begin{center}
\begin{small}
\begin{tabular}{p{0.1cm}c||c|c||c|c||c|c||}
\toprule
& & \multicolumn{2}{c||}{\textbf{CIFAR-10} Teacher Obj.} & \multicolumn{2}{c||}{\textbf{CIFAR-100} Teacher Obj.} & \multicolumn{2}{c||}{\textbf{TinyImageNet} Teacher Obj.} \\
% & & \multicolumn{2}{c||}{Teacher Obj.} & \multicolumn{2}{c||}{Teacher Obj.} & \multicolumn{2}{c||}{Teacher Obj.}\\
& & $L^{\std}$ & $L^{\rob}$ & $L^{\std}$ & $L^{\rob}$ & $L^{\std}$ & $L^{\rob}$ \\
\midrule
\multirow{10}{*}{\rotatebox{90}{Student Obj.}} 
& none & $86.48$ \tiny{$\pm 0.32$}  & $90.09 $ \tiny{$\pm 0.22$} &  $42.22 $ \tiny{$\pm 0.90$}  & $43.42 $ \tiny{$\pm 1.03$}  & $10.77 $ \tiny{$\pm 2.30$}  & $16.30 $ \tiny{$\pm 1.81$}\\
& & \tiny{($93.74 \pm 0.05$)} & \tiny{($92.67 \pm 0.09$)} & \tiny{$72.42 \pm 0.16$} & \tiny{$68.81 \pm 0.11$} & \tiny{($58.64 \pm 0.16$)} & \tiny{($50.52 \pm 0.22$)}\\
\cline{2-8}
& Post & $88.60 $ \tiny{$\pm 0.35$}  & $87.95 $ \tiny{$\pm 0.42$} & $38.19 $ \tiny{$\pm 1.25$}  &  $37.92 $ \tiny{$\pm 0.94$} & $11.22 $ \tiny{$\pm 0.38$}  & $13.58 $ \tiny{$\pm 0.40$}\\
& shift & \tiny{$92.16 \pm 0.18$} & \tiny{$91.21 \pm 0.18$} & \tiny{$61.22 \pm 1.15$} & \tiny{$61.84 \pm 0.93$} & \tiny{$43.63 \pm 0.65$} & \tiny{$43.23 \pm 0.83$}\\
\cline{2-8}
% & Ada & $88.33\pm0.14$  & $89.96\pm0.44$ & $45.61\pm \text{n/a}$  & $48.94\pm \text{n/a}$ & TBA  & TBA\\
% & Alpha & \tiny{($94.31\pm0.01$)} & \tiny{($93.97\pm0.07$)} & \tiny{$71.85\pm \text{n/a}$} & \tiny{$71.54\pm \text{n/a}$} & \tiny{TBA} & \tiny{TBA}\\
% \cline{2-8}
% & Ada & $87.36$ \tiny{$\pm0.06$}  & $90.37$\tiny{$\pm0.26$} & $42.92$ \tiny{$\pm 1.67$}  & $44.41$ \tiny{$\pm 0.82$} & \cellcolor{blue!25} $\mathbf{20.94}$ \tiny{$\pm 1.33$}  & $19.7$ \tiny{$\pm 1.24$}\\
% & Margin & \tiny{($94.25\pm0.02$)} & \tiny{($94.02\pm0.12$)} & \tiny{($73.88\pm 0.06$)} & \tiny{($70.49\pm 0.22$)} & \cellcolor{blue!25} \tiny{($58.46 \pm 0.12$)} & \tiny{($55.11 \pm 0.18$)}\\
% \cline{2-8}
& $L^{\stdd}$ & $87.66 $ \tiny{$\pm 0.40$}  & $90.12 $ \tiny{$\pm 0.23$}  & $43.81\pm0.58$  & \cellcolor{blue!25}$\mathbf{45.33}$ \tiny{$\pm0.82$} & $4.21 $ \tiny{$\pm 1.76$}  & $10.53 $ \tiny{$\pm 1.48$}\\
& & \tiny{($94.34 \pm 0.07$)} & \tiny{($94.07 \pm 0.07$)} & \tiny{$74.61\pm0.15$} & \cellcolor{blue!25}\tiny{$73.67\pm0.05$} & \tiny{($59.66 \pm 0.18$)} & \tiny{($56.55 \pm 0.15$)}\\
\cline{2-8}
& $L^{\robd}$  & \cellcolor{blue!25} $\mathbf{90.94} $ \tiny{$\pm 0.16$} & $85.14 $ \tiny{$\pm 0.47$} & $42.96$ \tiny{$\pm0.99$}  & $27.59\pm0.86$ & ${17.75} $ \tiny{$\pm 1.19$} & $6.00 $ \tiny{$\pm 1.65$}\\
&\tiny{(teacher val)} & \cellcolor{blue!25}\tiny{($92.54 \pm 0.05$)} & \tiny{($89.58 \pm 0.11$)} & \tiny{($68.71\pm0.15$)} & \tiny{($54.79\pm0.23$)} & \tiny{($47.81 \pm 0.13$)} & \tiny{($39.49 \pm 0.14$)}\\
\cline{2-8}
& $L^{\robd}$ & $89.37 $ \tiny{$\pm 0.17$} & $87.32 $ \tiny{$\pm 0.21$} & $40.36$ \tiny{$\pm 0.72$}  & $42.68\pm0.74$ & $14.70 $ \tiny{$\pm 1.65$} & $16.16 $ \tiny{$\pm 1.42$}\\
&\tiny{(one-hot val)} & \tiny{($91.63 \pm 0.06$)} & \tiny{($91.16 \pm 0.10$)} & \tiny{($61.49\pm0.22$)} & \tiny{($62.03\pm0.24$)} & \tiny{($50.16 \pm 0.18$)} & \tiny{($44.39 \pm 0.23$)} \\
\bottomrule
\end{tabular}

\begin{tabular}{p{0.1cm}c||c|c|c||c|c|c||}
\toprule
& & \multicolumn{3}{c||}{\textbf{CIFAR-10-LT} Teacher Obj.} & \multicolumn{3}{c||}{\textbf{CIFAR-100-LT} Teacher Obj.} \\
% & & \multicolumn{3}{c||}{Teacher Obj.} & \multicolumn{3}{c||}{Teacher Obj.} \\
& & $L^{\std}$ & $L^{\bal}$ & $L^{\rob}$ & $L^{\std}$ & $L^{\bal}$ & $L^{\rob}$ \\
\midrule
\multirow{14}{*}{\rotatebox{90}{Student Obj.}} 
& none & $57.26 $ \tiny{$\pm 0.55$} & $68.52 $ \tiny{$\pm 0.52$} & $74.8 $ \tiny{$\pm 0.30$} &   $0.00 $ \tiny{$\pm 0.00$} & $3.75 $ \tiny{$\pm 0.62$} & $10.33 $ \tiny{$\pm 0.82$} \\
&& \tiny{($76.27 \pm 0.20$)} & \tiny{($79.85 \pm 0.20$)} & \tiny{($80.29 \pm 0.12$)}  & \tiny{($43.33 \pm 0.16$)} & \tiny{($47.55 \pm 0.17$)} & \tiny{($44.27 \pm 0.13$)}\\
\cline{2-8}
& Post & $74.33 $ \tiny{$\pm 0.27$} & $73.60 $ \tiny{$\pm 0.46$} & $73.93 $ \tiny{$\pm 0.35$} &   $6.28 $ \tiny{$\pm 0.84$} & $8.89 $ \tiny{$\pm 0.69$} & $10.01 $ \tiny{$\pm 0.72$} \\
& shift & \tiny{($78.28 \pm 0.15$)}  & \tiny{($77.92 \pm 0.19$)} & \tiny{($77.93 \pm 0.12$)} &  \tiny{($27.93 \pm 0.46$)} & \tiny{($28.70 \pm 0.38$)} & \tiny{($29.88 \pm 0.61$)}\\
\cline{2-8}
& Ada & $47.52 $ \tiny{$\pm0.95$} & $66.74 $ \tiny{$\pm0.35$} & $70.33 $ \tiny{$\pm0.50$} & $0.00  $ \tiny{$\pm 0.00$} & $0.00  $ \tiny{$\pm 0.00$} & $12.46  $ \tiny{$\pm 0.36$} \\
& Margin & \tiny{($72.69\pm0.24$)} & \tiny{($78.20\pm0.09$)} & \tiny{($78.87\pm0.12$)}  & \tiny{($31.26 \pm 0.21$)} & \tiny{($34.06 \pm 0.12$)} & \tiny{($42.90 \pm 0.07$)}\\
\cline{2-8}
% & Ada & $41.90\pm0.44$ & $66.23\pm0.39$ & $71.17\pm0.32$  & $0.00 \pm 0.00$ & $1.46 \pm 0.61$ & $9.15 \pm 0.54$ \\
% & Alpha & \tiny{($71.67\pm0.08$)} & \tiny{($77.87\pm0.16$)} & \tiny{($79.66\pm0.13$)}   & \tiny{($42.52 \pm 0.08$)} & \tiny{($45.44 \pm 0.14$)} & \tiny{($45.64 \pm 0.11$)}\\
% \cline{2-8}
& $L^{\stdd}$ & $36.67  $ \tiny{$\pm 0.28$} & $66.96  $ \tiny{$\pm 0.43$} & $71.15  $ \tiny{$\pm 0.24$} & $0.00  $ \tiny{$\pm 0.00$} & $2.39  $ \tiny{$\pm 0.24$} & $7.32  $ \tiny{$\pm 0.47$} \\
&&\tiny{($69.5 \pm 0.13$)} & \tiny{($79.25 \pm 0.10$)} & \tiny{($80.95 \pm 0.11$)}  &\tiny{($43.86 \pm 0.14$)} & \tiny{($48.95 \pm 0.15$)} & \tiny{($47.93 \pm 0.11$)}\\
\cline{2-8}
& $L^{\bald}$ & $71.23  $ \tiny{$\pm 0.44$} & $70.52  $ \tiny{$\pm 0.20$} & $72.96  $ \tiny{$\pm 0.53$} & $4.39  $ \tiny{$\pm 0.65$} & $7.08  $ \tiny{$\pm 0.80$} & $7.19  $ \tiny{$\pm 0.79$} \\
&& \tiny{($80.5 \pm 0.12$)} & \tiny{($81.12 \pm 0.08$)} & \tiny{($80.71 \pm 0.07$)} & \tiny{($50.4 \pm 0.11$)} & \tiny{($50.1 \pm 0.09$)} & \tiny{($47.51\pm 0.20$)}\\
\cline{2-8}
& $L^{\robd}$  & $63.85  $ \tiny{$\pm 0.21$}  & \cellcolor{blue!25}$\mathbf{75.56} $ \tiny{$\pm 0.19$} & $69.21  $ \tiny{$\pm 0.45$}  & $9.05  $ \tiny{$\pm 0.71$}  & $12.52  $ \tiny{$\pm 0.98$} & $10.32  $ \tiny{$\pm 0.76$} \\
& \tiny{(teacher val)} & \tiny{($76.81 \pm 0.08$)} & \cellcolor{blue!25}\tiny{($80.81\pm 0.08$)} & \tiny{($76.72 \pm 0.19$)} & \tiny{($33.75 \pm 0.10$)} & \tiny{($34.05 \pm 0.09$)} & \tiny{($36.83 \pm 0.15$)}\\
\cline{2-8}
& $L^{\robd}$  & $73.59  $ \tiny{$\pm 0.25$} & $75.43  $ \tiny{$\pm 0.38$} & $74.7  $ \tiny{$\pm 0.19$} & $12.28  $ \tiny{$\pm 0.46$} & $11.94  $ \tiny{$\pm 0.80$} & \cellcolor{blue!25}$\mathbf{13.18}  $ \tiny{$\pm 0.61$} \\
& \tiny{(one-hot val)} & \tiny{($77.92 \pm 0.05$)} & \tiny{($79.02 \pm 0.07$)} & \tiny{($77.99 \pm 0.10$} & \tiny{($30.79 \pm 0.18$)} & \tiny{($29.8 \pm 0.20$)} & \cellcolor{blue!25}\tiny{($31.88 \pm 0.20$}\\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\vskip -0.2in
\end{table*}

% Such applications of robust optimization for satisfying fairness constraints across subgroups have for the most part focused on smaller models in a standard classification setting with experiments on small datasets such as COMPAS, Adult, and other UCI datasets, but the performance of these robust and constrained optimization techniques have not been explored in the setting of large datasets and models that necessitate distillation and compression. 
\textbf{Datasets.} We evaluate each robust distillation objective across different image dataset benchmarks: (i) CIFAR-10, (ii) CIFAR-100 \cite{Krizhevsky09learningmultiple}, and (iii) TinyImageNet  (a subset of ImageNet with 200 classes; \citet{le2015tiny}). We also include long tailed versions of each dataset \cite{cui2019class}.
%: (iv) CIFAR-10-LT, (v) CIFAR-100-LT, (vi) TinyImageNet-LT .
Details on sampling the long tailed versions of the datasets 
and additional results on the full ImageNet dataset \citep{ILSVRC15} are given in Appendix \ref{app:experiment_details}.
%\textbf{Test/validation splits:} 
For all datasets, we randomly split the original default test set in half to create our validation set and test set. We use the same validation and test sets for the long-tailed training sets as we do for the original versions, following the convention in prior work \cite{menon2020long, narasimhan2021training}. 
%For the long tailed training sets, this simulates a scenario where the training data follows a long tailed distribution, but the test distribution of interest still comes from the original balanced data distribution. 
%Thus, for the long tailed experiments, the average accuracy on test is measured on a dataset with balanced classes.

\textbf{Architectures.}  We evaluate our distillation protocols in both a self-distillation and compression setting. On all CIFAR datasets, all teachers were trained with the ResNet-56 architecture and students were trained with either ResNet-56 or ResNet-32. 
On TinyImageNet, teachers and students were trained with ResNet-18.
On ImageNet, teachers and students were trained with ResNet-34 and ResNet-18. 
This is as done by \citet{lukasik2021teachers} and \citet{he2016deep}, where more details on these architectures can be found (see, e.g., Table 7 in \citet{lukasik2021teachers}).

\textbf{Hyperparameters.} 
We apply temperature scaling to the teacher score distributions, i.e., compute $p^t(x) = \softmax(f^t(x) / \gamma)$, and  vary the temperature parameter $\gamma$  over a range of $\{1, 3, 5\}$.
Unless otherwise specified, the temperature hyperparameters were chosen to achieve the best worst-class accuracy on the validation set. A higher temperature produces a softer probability distribution over classes \citep{Hinton2015DistillingTK}. 
When teacher labels are applied to the validation set (see Section \ref{sec:algorithms}), we additionally include a temperature of 0.1 to approximate a hard thresholding of the teacher probabilities. We closely mimic the learning rate and regularization settings from prior work \cite{menon2020long,narasimhan2021training}. In keeping with the theory, the regularization ensures that the losses are bounded. 
See Appendix \ref{app:experiment_details} for further details.
%includes additional details about the training protocol.

\textbf{Baselines.}
We compare the robust distillation objectives with the following: 
% \vspace{-5pt}
% \begin{enumerate}[label=(\roman*),itemsep=0pt,topsep=0pt,leftmargin=16pt,nolistsep]
% \item \textbf{No distillation:} Models trained without distillation using each objective: $L^{\std}$, $L^{\bal}$, and $L^{\rob}$. We also include a comparison to group DRO \cite{Sagawa2020Distributionally} without distillation in Appendix \ref{app:experiment_details}, which differs from our robust objective $L^{\rob}$ in that our $L^{\rob}$ applies a margin-based loss.
% %We include the robust objective for this non-distilled model to illustrate any gains obtained from simply applying robust optimization without distillation.
% \item \textbf{Standard distillation without robustness:} Standard distillation protocol where both the teacher and student are trained with $L^{\std}$, $L^{\stdd}$, respectively.
% \item \textbf{Post-shifting:} 
% Following Section \ref{sec:theory}, we evaluate a post-shift approach
% that directly constructs a new scoring model by making post-hoc adjustments to the teacher,
% so as to maximize the robust accuracy on the validation sample \citep{narasimhan2021training}.
% % In section \ref{sec:post-hoc-adjustment}, we asked why not directly construct a new scoring model by making post-hoc adjustments
% % to the teacher? Here, we evaluate this strategy by applying the post-shifting in \citet{narasimhan2021training}. The post-shift coefficients are chosen to maximize the robust accuracy on the validation sample.
% % % ask whether it is a viable rough estimate of the worst-case performance that a student can hope to 
% % % achieve when using a particular teacher.
% \item \textbf{AdaMargin and AdaAlpha \citep{lukasik2021teachers}:}
% % This mitigation technique proposes a class specific weight that mixes a weighted combination of teacher
% % prediction and the true one-hot labels,
% % with the weights chosen using the validation set. 
% %When the weight is high, the student leans more heavily unto the one-hot training labels themselves. 
% % \todo{@Michal: can you add a bit of description discussing the difference between adamargin and adaalpha?}
% Both Ada* techniques are motivated by the observation that the margin defined by $\gamma_{\rm avg}( y, p^{\rm t}( x ) ) = p^{\rm t}_y( x ) - \frac{1}{m - 1} \sum_{y' \neq y} p^{\rm t}_{y'}( x )$ and averaged over examples from a particular class correlates with whether distillation improves over one-hot training \cite{lukasik2021teachers}. 
% AdaMargin uses that quantity as a margin in the distillation loss, whereas AdaAlpha uses it to adaptively mix between the one-hot and distillation losses.
% %We include comparisons to AdaMargin in the main paper, and include comparison to AdaAlpha in Table \ref{tab:adaalpha} in the Appendix, which achieves comparable performance.
% \end{enumerate}
% % \vspace{-5pt}
\textit{(i)} \textbf{No distillation:} Models trained without distillation using each objective: $L^{\std}$, $L^{\bal}$, and $L^{\rob}$. We also include a comparison to group DRO \cite{Sagawa2020Distributionally} without distillation in Appendix \ref{app:experiment_details} which differs from our robust objective $L^{\rob}$ in that we apply a margin-based loss with a validation set.
\textit{(ii)} \textbf{Standard distillation without robustness:} Standard distillation protocol where both the teacher and student are trained with $L^{\std}$, $L^{\stdd}$, respectively.
\textit{(iii)} \textbf{Post-shifting:} 
Following Section \ref{sec:theory}, we evaluate a post-shift approach
that directly constructs a new scoring model by making post-hoc adjustments to the teacher,
so as to maximize the robust accuracy on the validation sample \citep{narasimhan2021training}.
% In section \ref{sec:post-hoc-adjustment}, we asked why not directly construct a new scoring model by making post-hoc adjustments
% to the teacher? Here, we evaluate this strategy by applying the post-shifting in \citet{narasimhan2021training}. The post-shift coefficients are chosen to maximize the robust accuracy on the validation sample.
% % ask whether it is a viable rough estimate of the worst-case performance that a student can hope to 
% % achieve when using a particular teacher.
\textit{(iv)} \textbf{AdaMargin and AdaAlpha \citep{lukasik2021teachers}:}
% This mitigation technique proposes a class specific weight that mixes a weighted combination of teacher
% prediction and the true one-hot labels,
% with the weights chosen using the validation set. 
%When the weight is high, the student leans more heavily unto the one-hot training labels themselves. 
% \todo{@Michal: can you add a bit of description discussing the difference between adamargin and adaalpha?}
Both Ada* techniques are motivated by the observation that the margin defined for each class $y$ by $\gamma_{\rm avg}( y, p^{\rm t}( x ) ) = p^{\rm t}_y( x ) - \frac{1}{m - 1} \sum_{y' \neq y} p^{\rm t}_{y'}( x )$ %and averaged over examples from a particular class 
correlates with whether distillation improves over one-hot training \cite{lukasik2021teachers}. 
AdaMargin uses that quantity as a margin in the distillation loss, whereas AdaAlpha uses it to adaptively mix between the one-hot and distillation losses.
%We include comparisons to AdaMargin in the main paper, and include comparison to AdaAlpha in Table \ref{tab:adaalpha} in the Appendix, which achieves comparable performance.
% \vspace{-5pt}


\textbf{Which teacher/student combo is most robust?} %Results for worst-class accuracy: Which teacher-student combo is most robust?
For each objective and baseline,
we report the \textit{standard accuracy} over the test set (see \eqref{eq:std}), as well as the \textit{worst-class accuracy}, which we define to be the minimum per-class recall over all classes (see \eqref{eq:robust}). 
% For the long-tail datasets, note that as per the convention in 
% \citet{menon2020long}, the test sets are balanced over classes, so the standard accuracy over the test set is equivalent in distribution to the \textit{balanced accuracy} (see \eqref{eq:balanced}) over the long-tailed distribution.
For the long-tail datasets, we follow the convention in 
\citet{menon2020long} of reporting \textit{balanced accuracy} (see \eqref{eq:balanced}) instead of standard
accuracy. 
In each case, we use the 0-1 loss for evaluation.
Table \ref{tab:combos} shows results for various combinations of the proposed robust objectives and baselines.
%(more ImageNet results in Appendix \ref{app:tables}).
Across all datasets, the combination with best worst-class objective had at least one of either the teacher or the student apply the robust objective ($L^{\rob}$ or $L^{\robd}$). These combinations also achieve higher worst-class accuracy compared to the post-shift and AdaMargin techniques; although pairing these techniques with robust teachers could be competitive. Interestingly, post-shift was often seen to over-fit to the validation set, resulting in poorer test performance. 
As another comparison point, prior work by \cite{narasimhan2021training} also perform distillation with a standard teacher ($L^{\std}$) and robust student ($L^{\rob}$) with true one-hot labels on the validation set. In comparison to this, the new set of proposed robust combinations still achieves gains.

An inspection of the first row of Table \ref{tab:combos} reveals counter-intuitively that the teacher's worst-class accuracy is not a direct predictor of the robustness of a subsequent student. This couples with our theoretical understanding in Section \ref{sec:theory}, which showed that the ability of a teacher to train good students is determined by the calibration of scores within each class.
%For example, even if a teacher always predicts extremely low scores for a rare class and thus never ultimately classifies examples as belong to this class, this teacher may still train students with high accuracy on the rare class as long as the teacher's low scores are well-calibrated within the class.  
%
Perhaps surprisingly, it did not always benefit the robust student ($L^{\robd}$) to utilize the true one-hot labels in the validation set. Instead, training the robust student with teacher labels on the validation set was sufficient to achieve the best worst-class performance. This is promising from a data efficiency standpoint, since it can be expensive to build up a labeled dataset for validation, especially if the training data is long-tailed.


\begin{figure*}[t]
\vskip -0.2in
\begin{center}
\begin{tabular}{ccc}
    % & \tiny{CIFAR-10-LT (ResNet-56 $\to$ ResNet-32)} & \tiny{CIFAR-100-LT (ResNet-56 $\to$ ResNet-32)} \\
    \includegraphics[trim={2.8cm 0 2.8cm 0},clip,width=0.11\textwidth]{figures/legend_cf10lt_arch32_onehot.pdf} & \includegraphics[trim={0 0.2cm 0 0.1cm},clip,width=0.4\textwidth]{figures/plot_cf10lt_arch32_onehot} & \includegraphics[trim={0 0.2cm 0 0.1cm},clip,width=0.415\textwidth]{figures/plot_cf100lt_arch32_onehot}
\end{tabular}
\vspace{-5pt}
\caption{Trade-offs in worst-class test accuracy vs. balanced test accuracy for CIFAR-10-LT \textit{(left)} and CIFAR-100-LT \textit{(right)}, with ResNet-56 teachers and ResNet-32 students trained with one-hot validation labels. 
%Each point represents the outcome of a given combination of teacher/student objectives (with robustness tuned by $\alpha^t$ and $\alpha^s$, respectively in Eq. (\ref{eq:trade-off-distilled})), and points in the upper right are Pareto efficient. 
%For example, for CIFAR-10-LT, all of the Pareto optimal points were achieved when the teacher's loss used $\alpha^t = 0$ and the student's loss used $\alpha^s = 0.25$. 
Robust teacher/student combinations produce points that are more Pareto efficient than the ResNet-56 teachers alone. Additional plots in Appendix \ref{app:tradeoff_plots} show similar results for self distillation and teacher validation labels. Mean test performance over 10 runs is shown.
%, and all temperatures are included.
}
\label{fig:tradeoffs_cf-lt_32_onehot}
\end{center}
\vskip -0.3in
\end{figure*}

% Supplementing the analysis of worst-class accuracy, 
\textbf{Trading off balanced vs. worst-class accuracy.} We also evaluate the robust objectives in a setting where distillation is used for efficiency gains by distilling a larger teacher into a smaller student.
In Figure \ref{fig:tradeoffs_cf-lt_32_onehot}, we plot the full trade-off between balanced accuracy and worst-class accuracy for the robust distillation protocols. Each point represents the outcome of a given combination of teacher and student objectives, where the teacher optimizes $L^{\tdf}$ with tradeoff parameter $\alpha^t$, and the student optimizes $L^{\tdfd}$ with tradeoff parameter $\alpha^s$.  
%where $\alpha=0$ corresponds to minimizing average error ($L^{\bal}$), and $\alpha=1.0$ corresponds to minimizing worst-class error ($L^{\rob}$). 
Strikingly, Figure \ref{fig:tradeoffs_cf-lt_32_onehot} shows that ResNet-32 students distilled with robust trade-offs can be more Pareto efficient than even the larger ResNet-56 teacher models. Thus, distillation with combinations of robust losses not only helps worst-case accuracy, but also achieves better trade-offs with balanced accuracy. Similar trends prevail across our experiment setups, including self distillation and the original non-long-tailed datasets (see Appendix \ref{app:experiment_details}).

Overall, we demonstrate empirically and theoretically the value of applying different combinations of teacher-student objectives, not only for improving worst-class accuracy, but also to achieve efficient trade-offs between average and worst-class accuracy.  
Future avenues for exploration include experiments with mixtures of label types and effects of properties of the data on robustness.

% \textbf{Conclusion.} We demonstrate empirically and theoretically the value of applying robust optimization objectives for both the teacher and student, not only for improving worst-class accuracy, but more generally to achieve an efficient trade-off between average and worst-class accuracy. As future work, while we focus on training objectives, properties of the data can influence the efficiency and robustness of the distillation process as well, and warrants further exploration.

% \textbf{Conclusion and Future work.} 
% We demonstrate emprically and theoretically the value of applying robust optimization objectives for both the teacher and student, not only for improving worst-class accuracy, but more generally to achieve an efficient trade-off between average and worst-class accuracy.
% While our theory focuses on the properties of a teacher that yield robust students, further theoretical analysis of the efficiency/robustness trade-off for the student would be practically valuable. 
% % Further empirical study of a more general setting where students are trained with a mixture of teacher labels and one-hot labels would also be valuable. 
% Also, while we focus on training objectives, properties of the data can influence the efficiency and robustness of the distillation process as well, and also warrants further exploration.

% \textbf{Conclusion.}
% We demonstrate the value of applying robust optimization objectives for both the teacher and student, not only for the purpose of improving worst-class accuracy, but more generally to achieve an efficient tradeoff between average and worst-class accuracy. Our theoretical analysis further characterizes properties of the interaction between the teacher and student, and is supported by the empirical evidence that the most robust students don't always come from the most robust teachers. These insights can help guide the choice of distillation protocols in practice, especially when policy concerns do not allow for ignoring long tail classes.
% While our theory currently focuses on the properties of a teacher that yield robust students, further theoretical treatment of the efficiency/robustness tradeoff for the student would be practically valuable. 
% Our methods are extensible to a more general setting where students are trained with a weighted combination of data with teacher labels and one-hot labels, and further empirical study of this would be warranted. Finally, while we focus on training objectives, properties of the data can influence the efficiency and robustness of the distillation process as well, and also warrants further exploration.

==> robust-distillation (1)/intro.tex <==
\section{Introduction}
\label{sec:intro}


Knowledge distillation, wherein one trains a teacher model and uses its predictions to train a student model
of similar or smaller capacity, has proven to be a powerful tool that improves efficiency while achieving state-of-the-art classification accuracies on a variety of problems \citep{Hinton:2015, Radosavovic:2018, pham2021meta,46642,NEURIPS2020_3f5ee243}. While originally devised for model compression, distillation has also been widely applied to improve the performance of 
fixed capacity models and in semi-supervised learning settings \citep{rusu2016policy, Furlanello2018BornAN, yang2019training, xie2020self}. 

Evaluating the trade-offs incurred by distillation techniques has largely focused on canonical measures such as average error over a given data distribution. Along this dimension, distillation has proven to be a remarkably effective %compression 
technique, with the student achieving even better test performance than the teacher (e.g.\ \citet{xie2020self}). 
However, average error may differ significantly from the performance on individual subpopulations in the data, and thus may be an inadequate metric to optimize in real-world settings that also require good performance on different subgroups. For instance, subgroups may be defined by attributes such as country, language, or racial attributes \citep{Hardt:2016, zafar2017fairness, agarwal2018reductions}, in which case performance on the individual subgroups becomes a policy and fairness concern. % In a multi-class classification setting, each target class may be regarded a separate subgroup.

The potential for mismatch between average error and worst-group error is further exacerbated by the fact that many real-world datasets exhibit imbalance in the number of training examples belonging to different subgroups. In a multi-class classification setting where each target label delineates a subgroup, many real-world datasets exhibit a \textit{long-tailed} label distribution \citep{VanHorn:2017,menon2020long,feldman2021does,d2021tale}. Recent work has shown that improved average error of the student model often comes at the expense of poorer performance on the tail classes \cite{lukasik2021teachers,du2021compressed}
or under-represented groups \citep{sagawa2020investigation, menon2020overparameterisation}, and model compression can amplify performance disparities across groups \cite{hooker2020characterising, xu-etal-2021-beyond}. Further hurting test performance is the possibility that the training data may have particularly poor representation of important subgroups that occur more frequently at deployment or test time.
%This distribution shift may be due to bias in training data collection and labeling.robust optimization

% To address this goal of achieving good worst-case performance across subgroups in a standard single model training setting, 
To mitigate the disparity between average error and subgroup performance, a common approach is to train a model to achieve low worst-group test error. Modified objectives for robust optimization techniques have successfully achieved state-of-the-art worst-class performance with manageable computational overhead \citep{Sagawa2020Distributionally, sohoni2020no, narasimhan2021training}. However, an evaluation of these techniques has disproportionately focused on a standard single model training setting. 
In this work, we focus on applying robust optimization to a multi-step training setting typical of distillation. We take a wider view of the optimization process, and ask what combination of student and teacher objectives achieves low worst-group test error \emph{and} minimizes difference between average and worst case error. 

To integrate robust optimization objectives into the distillation procedure, we introduce a robust objective for either the teacher, the student, or both. We also quantify the trade-off between average error across all subgroups and the worst-group error by mapping out Pareto fronts for each distillation procedure.
Theoretically, we ask the question, \textit{what makes for a ``good'' teacher} when training a robust student? That is, what properties are important in a teacher so that a student achieves good worst-class performance?

In summary, we make the following contributions:
\begin{enumerate}[label=(\roman*),itemsep=0pt,topsep=0pt,leftmargin=16pt,nolistsep]
\item We present distillation techniques integrating distributionally robust optimization (DRO) algorithms with the goal of achieving a robust student, and explore different combinations of modifications to the teacher and student objectives. 
%\item We empirically compare these robust distillation algorithms for introducing robust optimization into distillation, exploring the tradeoff between overall performance and worst-class performance. We compare these to simpler baselines such as post-shifting and balancing the objective function.
\item In both self-distillation and compression settings, we empirically demonstrate that the proposed robust distillation algorithms can train student models that yield better worst-class accuracies than the teacher and other recent baselines. We also demonstrate gains in the trade-off between overall and worst-class performance.
% (when training students of similar capacity).
% We show that our robust objectives 
% also achieve better trade-offs between overall and worst-class performance compared to baselines such as post-shifting and simpler loss modifications.
\item We derive robustness guarantees for the student under  different algorithmic design choices, and % provide theoretical insights into what makes a ``good'' teacher when the goal is to train a robust student,
% and %derive robustness guarantees for the student in terms of the teacher's approximation errors.
provide  insights into when the student yields better worst-class robustness than the teacher.
% .  These serve as a framework for understanding the reasons behind the comparative performance of different algorithms, and can guide the development of future improvements on robust distillation algorithms.
\end{enumerate}


\textbf{Related Work.}\
\textit{Fairness in distillation:}\
% One of the most relevant prior work is 
\citet{lukasik2021teachers} study how distillation impacts worst-group performance and observe that the errors that the teacher makes on smaller subgroups get amplified and transferred to the student. They also propose simple modifications to the student's objective to control the strength of the teacher's labels for different groups. In contrast, in this work we propose a more direct and theoretically-grounded procedure that
seeks to explicitly optimize for the student's worst-case error, and explore modifications to both the teacher and student objectives. 


\textit{Worst-group robustness:}\ The goal of achieving good worst-case performance across subgroups can be framed as a 
(group) distributionally robust optimization (DRO) problem, 
and can be solved by iteratively updating costs on the individual groups and minimizing the resulting cost-weighted loss \citep{chen2017robust}. Recent variants of this approach have sought to avoid over-fitting through
group-specific regularization \citep{Sagawa2020Distributionally} or
margin-based losses \cite{narasimhan2021training, kini2021labelimbalanced},
to handle unknown subgroups \citep{sohoni2020no}, and to balance between average and worst-case performance \cite{piratla2021focus}. Other approaches include the use of Conditional Value at Risk for worst-class robustness \citep{xu2020class}.

Among these, the work that most closely relates to our paper
is the margin-based DRO algorithm \citep{narasimhan2021training}, 
which includes preliminary distillation experiments in support of training the teacher with
standard ERM and the student with a robust objective. 
However, this and other prior work have only explored modifications to the student loss \cite{lukasik2021teachers,narasimhan2021training}, while training the teacher using a standard procedure.
{Our robust distillation proposals build on this method,
but carry out a more extensive analysis, exploring different combinations of teacher-student objectives 
and different trade-offs between average and worst-class performance}. Additionally,
we provide robustness guarantees for the student, equip the DRO algorithms to achieve different trade-offs between overall and worst-case error, and provide a rigorous analysis of different design choices.


==> robust-distillation (1)/preamble.tex <==
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\cO}{\mathcal{O}}

\newcommand{\1}{\mathbf{1}}
\renewcommand{\>}{\rightarrow}
\newcommand{\E}{\mathbb{E}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\boldf}{\mathbf{f}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\blambda}{{\lambda}}

\newcommand{\bV}{\mathbb{V}}
\newcommand{\cM}{\mathcal{M}}

\newcommand{\Argmax}[1]{\underset{#1}{\operatorname{argmax}}}
\newcommand{\Argmin}[1]{\underset{#1}{\operatorname{argmin}}}
\newcommand{\argmax}[1]{{\operatorname{argmax}}_{#1}}
\newcommand{\argmin}[1]{{\operatorname{argmin}}_{#1}}


\newcommand{\err}{\textrm{\textup{ERR}}}
\newcommand{\wer}{\textrm{\textup{WER}}}
\newcommand{\ber}{\textrm{\textup{BER}}}
\newcommand{\val}{\textrm{\textup{val}}}


\newcommand{\xent}{\textrm{\textup{xent}}}
\newcommand{\dis}{\textrm{\textup{dis}}}
\newcommand{\bal}{\textrm{\textup{bal}}}
\newcommand{\wc}{\textrm{\textup{wor}}}
\newcommand{\rob}{\textrm{\textup{rob}}}
\newcommand{\robd}{\textrm{\textup{rob-d}}}
\newcommand{\bald}{\textrm{\textup{bal-d}}}
\newcommand{\zo}{\textrm{\textup{0-1}}}
\newcommand{\std}{\textrm{\textup{std}}}
\newcommand{\stdd}{\textrm{\textup{std-d}}}
\newcommand{\tdf}{\textrm{\textup{tdf}}}
\newcommand{\tdfd}{\textrm{\textup{tdf-d}}}
\newcommand{\mar}{\textrm{\textup{mar}}}
\newcommand{\oh}{\textrm{\textup{oh}}}
\newcommand{\softmax}{\textrm{\textup{softmax}}}

\newcommand\AddLabel[1]{\refstepcounter{equation}(\theequation)\label{#1}}

% To control spacing in itemized lists
\usepackage{enumitem}

% Algorithm command
\usepackage{algorithm}
\usepackage{algorithmic} 

% Theorems
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

% Todonotes is useful during development; simply uncomment the next line
%    and comment out the line below the next line to turn off comments
%\usepackage[disable,textsize=tiny]{todonotes}
\usepackage[textsize=tiny]{todonotes}


==> robust-distillation (1)/prelims.tex <==
\section{Problem Setup}
\label{sec:prelims}

We are interested in a multi-class classification problem with instance space $\X$
and output space $[m] = \{1, \ldots, m\}$. Let $D$ denote the underlying data distribution over $\X \times [m]$, and 
$D_{\X}$ denote the marginal distribution over $\X$.
Let $\Delta_m$ denote the $(m-1)$-dimensional probability simplex over $m$ classes. 
We define the
conditional-class probability as $\eta_y(x) = \P(Y=y|X=x)$ and the class priors $\pi_y = \P(Y=y)$.
Note that $\pi_y = \E_{X \sim D_\X}\left[ \eta_y(X) \right]$. 

\textbf{Learning objectives.}
Our goal is to learn a multiclass classifier $h: \X \> [m]$ that maps an instance $x \in \X$ to one of $m$ classes.
We will do so by first learning a scoring function $f: \X \> \R^m$ that assigns scores $[f_1(x), \ldots, f_m(x)] \in \R^m$  to a given instance $x$,
and construct the classifier by predicting the class with the highest score: $h(x) = \argmax{j \in [m]}\,f_j(x)$. We will 
%compute confidence scores or probabilities by applying a
denote a softmax transformation of $f$ by $\softmax_y(f(x)) = \frac{\exp( f_y(x) ) }{\sum_j \exp( f_j(x) )}$,
and use the notation  $\softmax_y(f(x)) \propto z_y$ to indicate that $\softmax_y(f(x)) = \frac{z_y}{\sum_{j=1}^m z_j}$.

We measure the efficacy of the scoring function $f$ using a loss function $\ell: [m] \times \R^m \> \R_+$
that assigns a penalty $\ell(y, z)$ for predicting score vector $z \in \R^m$ for true label $y$. Examples of loss functions include the 
0-1 loss: $\ell^\zo(y, z) = \1\left(z \ne \argmax{j}\,f_j(x) \right)$,
% \begin{align}
% \ell^\zo(y, z) = \1\left(z \ne \argmax{j}\,f_j(x) \right),
% \label{eq:0-1}
% \end{align}
and the softmax cross-entropy loss: $\ell^\xent(y, z) = \textstyle -f_y(x) + \log\big( \sum_{j \in [m]} \exp\left( f_j(x) \right) \big)$.
% \begin{align}
% \ell^\xent(y, z) = \textstyle -f_y(x) + \log\left( \sum_{j \in [m]} \exp\left( f_j(x) \right) \right).
% \label{eq:xent}
% \end{align}

\textit{Standard objective:} A standard machine learning goal entails minimizing the overall expected risk: 
%This is reflected in the objective:
\begin{equation}
L^\std(f) = \E\left[\ell(Y, f(X))\right].
\label{eq:std}
\end{equation}
% In a standard setup, one often picks the classifier $h$ to minimize the expected 0-1 error:
% \[
% \err(h) = \E\left[\1(h(X) \ne Y)\right].
% \]
% Because this objective is non-continuous in $h(X)$, a common proxy is to
% pick a scoring function $f$ that minimizes the expected cross-entropy loss:
% One often chooses a scoring function $f$ that minimizes a 
% \begin{align}
% L^\std(f) = \E\left[\ell(Y, f(X))\right],
% \label{eq:std}
% \end{align}
% where $\ell: [m] \times \R^m \> \R_+$ is a loss function, 
% and to construct a classifier from the minimizer $f^*$ using: $h^*(x) = \argmax{i \in [m]}\,f^*_i(x)$.
%which we will refer to as the \emph{standard} objective.
%
\textit{Balanced objective:} In applications where the classes are severely imbalanced, i.e.,
the class priors $\pi_y$ are non-uniform and significantly skewed,
one may wish to instead optimize a \emph{balanced} version of the above objective,
where we average over the conditional loss for each class. Notice that  the
conditional loss for class $y$ is weighted by the inverse of its prior:
\allowdisplaybreaks
\begin{align}
    L^\bal(f) %&= \max_{y \in [m]} \frac{1}{\pi_y}\E_{x, y}\left[ \ell(y, f(x)) \right], \nonumber\\
            % &= \max_{y \in [m]} \frac{1}{\pi_y}\E_{X,Y}\left[\mathbf{1}(Y=y)\ell(Y, f(X))\right]\nonumber\\
            &= \frac{1}{m}\sum_{y \in [m]} \E\left[\ell(y, f(X))\,|\, Y = y \right]
            % \nonumber\\
            % ~=~ \frac{1}{m}\sum_{y \in [m]}  \frac{1}{\P(Y=y)}\E_{X, Y}\left[\1(Y=y)\ell(y, f(X))\right]\nonumber\\
         ~=~ \frac{1}{m}\sum_{y \in [m]}  \frac{1}{\pi_y}\E_X\left[ \eta_y(X)\,\ell(y, f(X)) \right].
    \label{eq:balanced}
\end{align}
%
\textit{Robust objective:} A more stringent objective would be to focus on the worst-performing class, and 
minimize a \emph{robust} version of
 \eqref{eq:std} that computes
the worst among the $m$
conditional losses:
% \[
% \wer(h) = \max_{y \in [m]} \E\left[\1(h(X) \ne y) \,|\, Y = y\right].
% \]
% As a proxy for this objective, we seek to learn
% a scoring function that minimizes the following \emph{robust} version of \eqref{eq:std}:
\begin{align}
    L^\rob(f) %&= \max_{y \in [m]} \frac{1}{\pi_y}\E_{x, y}\left[ \ell(y, f(x)) \right], \nonumber\\
            % &= \max_{y \in [m]} \frac{1}{\pi_y}\E_{X,Y}\left[\mathbf{1}(Y=y)\ell(Y, f(X))\right]\nonumber\\
            % &= \max_{y \in [m]} \E\left[\ell(y, f(X))\,|\, Y = y \right]\nonumber\\
            % &= \max_{y \in [m]} \frac{1}{\P(Y=y)}\E\left[\1(Y=y)\ell(y, f(X))\right]\nonumber\\
         &= \max_{y \in [m]} \frac{1}{\pi_y}\E\left[ \eta_y(X)\,\ell(y, f(X)) \right].
    \label{eq:robust}
\end{align}
%which we will refer to as the \emph{robust} objective.
In practice, focusing solely on either the average or the worst-case performance may not 
be an acceptable solution, and therefore, in this paper, we will additionally seek to characterize the
trade-off between the balanced and robust objectives. One way to achieve this trade-off is to minimize the robust objective, while constraining the balanced objective to
be within an acceptable range. This constrained optimization can be equivalently formulated as optimizing a convex combination of the balanced and robust objectives, for trade-off %parameter 
$\alpha \in [0,1]$:
\begin{align}
    L^\tdf(f)
         &= (1 - \alpha) L^\bal(f) + \alpha L^\rob(f).
    \label{eq:trade-off}
\end{align}
 A similar trade-off can also be specified between the standard and robust objectives.
% A compromise between optimizing the overall error and the worst-case error may be
% to minimize the average conditional error, often referred to as \emph{balanced error rate}:
% \[
% \ber(h) = \frac{1}{m}\sum_{y \in [m]} \E\left[\1(h(X) \ne y) \,|\, Y = y\right],
% \]
% a proxy for which is given by the following \emph{balanced} loss:
% \begin{align}
%     L^\bal(f) %&= \max_{y \in [m]} \frac{1}{\pi_y}\E_{x, y}\left[ \ell(y, f(x)) \right], \nonumber\\
%             % &= \max_{y \in [m]} \frac{1}{\pi_y}\E_{X,Y}\left[\mathbf{1}(Y=y)\ell(Y, f(X))\right]\nonumber\\
%             % &= \max_{y \in [m]} \E\left[\ell(y, f(X))\,|\, Y = y \right]\nonumber\\
%             % &= \max_{y \in [m]} \frac{1}{\P(Y=y)}\E\left[\1(Y=y)\ell(y, f(X))\right]\nonumber\\
%          &= \frac{1}{m}\sum_{y \in [m]} \frac{1}{\pi_y}\E\left[ \eta_y(X)\,\ell(y, f(X)) \right].
%     \label{eq:balanced}
% \end{align}
%
%\textbf{Bayes-optimal scorers.} 
To better understand the differences between the standard, balanced and robust objectives in \eqref{eq:std}--\eqref{eq:trade-off},
we look at the optimal scoring function for each given a cross-entropy loss:
\begin{theorem}[\textbf{Bayes-optimal scorers}]
\label{thm:bayes}
When $\ell$ is %a proper-composite loss 
%that is strictly convex in its second argument (e.g., 
the cross-entropy loss $\ell^\xent$, %in \eqref{eq:xent},
the minimizers of \eqref{eq:std}--\eqref{eq:robust} over all measurable functions $f: \X \> \R^m$ are given
by:

\begin{tabular}{llll}
    \textit{(i)} $L^\std(f)$: &  $\softmax_y( f^{*}(x) ) \,=\, \eta_y(x)$ & \textit{(ii)} $L^\bal(f)$: &  $\softmax_y( f^{*}(x) ) \,\propto\, \frac{1}{\pi_y}\eta_y(x)$ \\
    \textit{(iii)} $L^\rob(f)$: & $\softmax_y( f^{*}(x) ) \,\propto\, \frac{\lambda_y}{\pi_y}\eta_y(x)$ & \textit{(iv)} $L^\tdf(f)$: & $\softmax_y( f^{*}(x) ) \,\propto\, \frac{(1 - \alpha)\frac{1}{m} + \alpha\lambda'_y}{\pi_y}\eta_y(x),$
\end{tabular}

% \begin{tabular}{ll}
%     \emph{(a)} $L^\std(f)$: &  $\softmax_y( f^{*}(x) ) \,=\, \eta_y(x)$ \\
%     \emph{(b)} $L^\bal(f)$: &  $\softmax_y( f^{*}(x) ) \,\propto\, \frac{1}{\pi_y}\eta_y(x)$ \\
%     \emph{(c)} $L^\rob(f)$: & $\softmax_y( f^{*}(x) ) \,\propto\, \frac{\lambda_y}{\pi_y}\eta_y(x)$\\
%     \emph{(d)} $L^\tdf(f)$: & $\softmax_y( f^{*}(x) ) \,\propto\, \frac{(1 - \alpha)\frac{1}{m} + \alpha\lambda'_y}{\pi_y}\eta_y(x),$
% \end{tabular}

% \begin{enumerate}
%     \item The minimizer of $L^\std(f)$ is given by $f^{*}_y(x) = \log(\eta_y(x))$;
%     \item The minimizer of $L^\bal(f)$ is given by $f^{*}_y(x) = C\log\left(\frac{1}{\pi_y}\eta_y(x)\right)$ for some constant $C > 0$;
%     \item The minimizer of $L^\rob(p)$ is given by $f^{*}_y(x) = C'\log\left(\frac{\lambda_y}{\pi_y}\eta(x)\right)$ for constant $C' > 0$.
% \end{enumerate}
for class-specific constants $\lambda, \lambda' \in \R^m_+$ that depend on distribution $D$.
\vspace{-5pt}
\end{theorem}

All proofs are provided in Appendix \ref{app:proofs}.
%The first result follows from the property of the cross-entropy loss \citep{williamson2016composite}; see \citet{menon2020long} for a proof of the second result; we provide a proof for the third and fourth results in Appendix \ref{app:proof-bayes}. 
Interestingly, the optimal scorers for all four objectives involve a simple scaling of the conditional-class probabilities $\eta_y(x)$.

% The form of the optimal scorers suggests the following alternate approach to optimizing the balanced objective $L^\bal$ and the robust objective $L^\rob$: first train a scoring function by minimizing the standard objective $L^\std$, and make post-hoc adjustments to its predictions to construct the optimal scorer for the balanced or robust objectives. This post-hoc approach is straight-forward to implement for the balanced objective, where one only needs an estimate of the class priors
% $\pi_y$ to perform the adjustment, and may be tricky for the robust objective, where the scaling post-hoc coefficients $\lambda_1, \ldots, \lambda_m$ needed are not known apriori. We will revisit this post-hoc adjustment strategy in the next section.

==> robust-distillation (1)/theory.tex <==
\section{Theoretical Analysis}
\label{sec:theory}
%Moving to our theoretical analysis, we would
% like to understand 
% what constitutes a good teacher and how it
% aids a student in achieving robustness. 
To simplify our exposition, we will present  our theoretical analysis 
for a student trained using Algorithm \ref{algo:dro} to yield good worst-class performance. Our results easily extend to the case where the student seeks to trade-off between overall and worst-case performance. 

\textbf{What constitutes a good teacher?}
%\label{sec:theory_good_teacher}
We would first like to understand what makes a good teacher 
when the student's goal is to minimize the robust population objective $L^\rob(f^s)$ in \eqref{eq:robust}. We also analyze whether the student's ability to perform well on this worst-case objective depends on
the teacher also performing well on the same objective.
%
As a proxy for $L^\rob(f^s)$, the
student minimizes the distilled objective $\hat{L}^\robd(f^s)$ in \eqref{eq:robust-distilled-empirical} 
with predictions from teacher $p^t$.
We argue that an \emph{ideal} teacher 
in this case
would be one that ensures that
the difference between the two objectives
$
|\hat{L}^\robd(f^s) - L^\rob(f^s)|
$
is as small as possible. Below, we provide a simple bound on this difference:
\begin{theorem}
\label{thm:good-teacher}
% Define population version of the student's objective in \eqref{eq:robust-distilled-empirical} as:
% \begin{align*}
%     {L}^\robd(f^s) &= \max_{y \in [m]} \frac{1}{\pi^t_y}\E_x\left[ p_y^t(x)\, \ell\left( y , f^s(x) \right)\right].\hspace{-5pt}
%     \label{eq:robust-distilled-population}
% \end{align*}
Suppose $\ell(y, z) \leq B, \forall x \in \X$ for some $B > 0$. 
Let $\pi^t_y = \E_x\left[ p_y^t(x) \right]$,
and let the following denote the per-class expected and empirical student losses respectively:
\begin{align*}
\phi_y(f^s) = \textstyle\frac{1}{\pi^t_y}\E_x\left[ p_y^t(x)\, \ell\left( y , f^s(x) \right)\right]; \quad \hat{\phi}_y(f^s) = \textstyle\frac{1}{\hat{\pi}^t_y}\frac{1}{n}\sum_{i=1}^n  p_y^t(x_i)\,\ell\left( y , f^s(x_i) \right).
\end{align*}
% \begin{align*}
% \phi_y(f^s) &= \textstyle\frac{1}{\pi^t_y}\E_x\left[ p_y^t(x)\, \ell\left( y , f^s(x) \right)\right]\\[-2pt]
% \hat{\phi}_y(f^s) &= \textstyle\frac{1}{\hat{\pi}^t_y}\frac{1}{n}\sum_{i=1}^n  p_y^t(x_i)\,\ell\left( y , f^s(x_i) \right).
% \end{align*}
Then for teacher $p^t$ and student $f^s$:
% for any $\delta \in (0,1)$,
% with probability $\leq 1 - \delta$ (over draw of $S$), 
% {\color{green}TBD: Derive $\Delta(n,\delta)$}
\begin{align*}
|\hat{L}^\robd(f^s) - L^\rob(f^s)|
&\leq
\underbrace{
    B\max_{y \in [m]} \E_x\left[
        \left| \frac{p^t_y(x)}{\pi^t_y} - \frac{\eta_y(x)}{\pi_y} \right|\right]}_{\text{Approximation error}}
+
\underbrace{
\max_{y \in [m]} \big|\phi_y(f^s) - \hat{\phi}_y(f^s)\big|}_{\text{Estimation error}}.
\end{align*}
% where $\pi^t_y = \E_x\left[p^t_y(x)\right]$.
% \vspace{-7pt}
\end{theorem}
%
% See Appendix \ref{app:proof-good-teacher} for the proof.
The \emph{approximation error} %in the above bound 
captures 
how well the teacher's predictions mimic the conditional-class distribution $\eta(x) \in \Delta_m$, 
up to per-class normalizations. 
This suggests that even if $p^t$ does not 
achieve good worst-class performance, as long as
it is well calibrated within each class (as measured by the approximation error above), 
it will serve as a good teacher. Indeed when the teacher outputs the conditional-class probabilities, 
i.e.\ $p^t(x) = \eta(x)$, the  approximation error is trivially zero (recall that the normalization term
$\pi^t_y = \pi_y$ in this case). We  know from
Theorem \ref{thm:bayes} that, this would be the case with a teacher
trained to optimize the standard cross-entropy objective (provided we use an unrestricted model class). 
In practice, however, we do not expect the teacher to approximate $\eta(x)$ very well,
and this opens the door for training the teacher with the other objectives described in Section \ref{sec:prelims}, each
of which encourage the teacher to approximate a scaled (normalized) version of $\eta(x)$.
% On the other hand, 
% it is not
% immediate if a teacher that optimizes the balanced or robust objectives
% will yield low approximation errors (as it is not clear what
% the normalization terms will evaluate to for them). %In our experiments, we probe further into the efficacies of these models as teachers.
% This is a  less stringent requirement on the teacher 
% compared to the condition in \citet{menon2021statistical}, where 
% the goal is to optimize the standard objective, and the teacher
% is evaluated based on how well it approximates the exact conditional probabilities $\eta(x)$.
% Consequently, any teacher of the form $p_y^t(x) = \alpha_y\eta_y(x)$, 
% for scaling factor $\alpha \in \R_+^m$, would yield an approximation error of zero. Note that
% this is indeed the case with each of the Bayes-optimal scorers in Theorem \ref{thm:bayes}. 
% This suggests that one can train a teacher by optimizing any of the objectives in \eqref{eq:std}--\eqref{eq:robust},
% apply a softmax transformation to them to predict probabilities, 
% and have the student optimize the distilled robust objective in \eqref{eq:robust-distilled-empirical} against
% the teacher's probabilities.\todo{This claim is not entirely correct when the teacher scores are normalized to sum to 1. TODO[Hari]: rephrase this!}

The \emph{estimation error} captures how well the teacher aids in the student's out-of-sample generalization. 
The prior work by \citet{menon2021statistical} studies  this question in detail for 
the standard student objective, and 
provide a bound that depends on the variance induced by the teacher's predictions on the
student's objective: the lower the variance, the better the student's generalization.
 A similar analysis can be carried out with the per-class loss terms in Theorem \ref{thm:good-teacher} (more details in Appendix \ref{app:student-gen-bound}).
%In Appendix \ref{app:gen-bound}, we extend results from \citet{menon2021statistical} to derive a uniform convergence bound on  $|\hat{L}^\robd(f) - L^\robd(f)|$ 
% in terms of the variance of the loss induced by the teacher's predictions. 
% The lower the variance the faster is the convergence of the empirical risk to the population risk.

% \begin{theorem}
% \textup{\color{green}TBD}
% \todo{Add generalization bound on $|\hat{L}^\robd(f) - L^\robd(f)|$}
% \vspace{2cm}
% \label{thm:gen-bound}
% \end{theorem}

% \vspace{-2pt}
\textbf{Robustness guarantee for the student.}\
% \todo{To be done}
%Having chosen a teacher model $p^t$, we would next like to understand the  form of the optimal student for $\hat{L}^\robd(f)$.
% (in the limit of infinite training samples).
We next seek to understand if the student can match or outperform the teacher's worst-class performance.
For a fixed teacher $p^t$, we
 consider a \emph{self-distillation} setup where 
the student is chosen from the same function class $\cF$ as the teacher,
and can thus exactly mimic the teacher's predictions.
Under this setup, 
we provide robustness gurarantees
for the student output by Algorithm \ref{algo:dro} 
in terms of the approximation and estimation errors
described above. %, and the convergence rate
%of the exponentiated gradient (EG) ascent algorithm. 

%We assume a fixed teacher $p^t$ and focus 
% on a \emph{self-distillation} setting where both
% the student and teacher are chosen from the same hypothesis class $\cF$. 
\begin{proposition}
\label{prop:student-form}
% For a fixed teacher $p^t: \X \> \Delta_m$, when $\ell$ is the cross-entropy loss,
% the minimizer of $\hat{L}^\robd(f)$ in \eqref{eq:robust-distilled-empirical} over all 
% measurable functions $f: \X \> \R^m$ is of the form:
% $$
% \softmax_y(f^*(x')) \propto \gamma_y p^t_y(x'),~~\forall (x', y') \in S,
% $$
%  for some class-specific constants $\gamma_1, \ldots, \gamma_m \in \R$.
Suppose $p^t \in \cF$ and $\cF$ is closed under linear transformations. Let $\bar{\lambda}_y = (\prod_{k=1}^K {\lambda_y^k}/{\pi^t_y})^{1/K}, \forall y$.
%, \forall y$. 
Then the scoring function $\bar{f}^s(x) = \frac{1}{K} \sum_{k=1}^K f^{k}(x)$ output by Alg. \ref{algo:dro} is of the form:
%is of the form:
% \vspace{3pt}
    \[
        \softmax_j(\bar{f}^s(x)) \propto \bar{\lambda}_j p_j^t(x),~\forall j \in [m],\, \forall (x, y) \in S.
    \]
% \vspace{2pt}
% where $\bar{\lambda}_j = \left(\prod_{k=1}^K {\lambda_j^k}/{\pi^t_j}\right)^{1/K}$. 
\end{proposition}
%
\begin{theorem}
\label{thm:dro}
Suppose $p^t \in \cF$ and $\cF$ is closed under linear transformations. 
Suppose
$\ell$ is the cross-entropy loss $\ell^{\xent}$,
$\ell(y, z) \leq B$
and $\max_{y \in [m]}\frac{1}{\pi^t_y} \leq Z$,
for some $B, Z > 0$. 
Furthermore, suppose for any $\delta \in (0,1)$, the following bound holds on the
estimation error in Theorem \ref{thm:good-teacher}:
with probability at least $1 - \delta$ (over draw of $S \sim D^n$),
$\forall f \in \cF$, $\textstyle
\max_{y \in [m]} \big|\phi_y(f) - \hat{\phi}_y(f)\big| \leq \Delta(n, \delta),$
% \[
% \textstyle
% \max_{y \in [m]} \big|\phi_y(f) - \hat{\phi}_y(f)\big| \leq \Delta(n, \delta),
% \]
for some $\Delta(n, \delta) \in \R_+$ that
is increasing in $1/\delta$, and goes to 0 as $n \> \infty$. 
Then when the step size $\gamma = \frac{1}{2BZ}\sqrt{\frac{\log(m)}{{K}}}$
and $n^\val \geq 8Z\log(2m/\delta)$, we have that with
probability at least $1-\delta$ (over draw of $S \sim D^n$ and $S^\val \sim D^{n^\val}$),
% \vspace{8pt}
\begin{align*}
\lefteqn{
L^\rob(\bar{f}^s) \,\leq\,
    \min_{f \in \cF}L^\rob(f)}
\\[-10pt]
 &\hspace{1cm}
 +\,
        \underbrace{2\Delta(n^\val, \delta/2) \,+\,  2\Delta(n, \delta/2)}_{\text{Estimation error}}
\,+\,
\underbrace{
2B\max_{y \in [m]} \E_x\left[
        \left| \frac{p^t_y(x)}{\pi^t_y} \,-\, \frac{\eta_y(x)}{\pi_y} \right|\right]}_{\text{Approximation error}}
        \,+\,
        \underbrace{4BZ\sqrt{\frac{\log(m)}{{K}}}}_{\text{EG convergence}}.
\end{align*}
\vspace{-10pt}
\end{theorem}


% The proof is provided in Appendix \ref{app:convergence-dro}, and 
% builds on the
% convergence guarantee for
% exponentiated gradient (EG) ascent \citep{shalev2011online}
% and calibration properties of the margin loss \citep{narasimhan2021training}. %Therefore when the student optimizes over e.g.\ an over-parameterized function class, %and has access to unlimited training data, 

% Theorem \ref{thm:dro}
Proposition \ref{prop:student-form} shows the student 
not only learns to mimic the teacher on the training set, but makes per-class adjustments to its predictions,
and Theorem \ref{thm:dro} shows that these adjustments are chosen to close-in on the
gap to the optimal robust scorer in $\cF$.
The form of the student
 suggests that it can not only match the teacher's performance,
but can potentially improve upon it by making %scaling 
adjustments to its scores. 
However, the student's convergence to the optimal scorer in $\cF$
would still be limited by the teacher's approximation error:
even when the sample sizes and number of iterations $n, n^\val, K \> \infty$,
the student's optimality gap may still be non-zero as long as the teacher is sub-optimal. 

\textbf{Connection to post-hoc adjustment.}\
%\label{sec:post-hoc-adjustment}
% \vspace{-2pt}
The form of the student %in the self-distillation setup 
in Proposition \ref{prop:student-form} raises an interesting question. Instead of training an explicit student model, 
why not directly construct a new scoring model by making post-hoc adjustments
to the teacher's predictions? Specifically, one could optimize over functions of the form $f^s_y(x) = \log(\gamma_y p^t_y(x)),$ where the teacher $p^t$ is fixed, and pick 
the coefficients $\gamma \in \R^m$ so that resulting scoring function yields the best worst-class accuracy on a held-out dataset.  
This simple \emph{post-hoc adjustment} strategy 
may not be feasible if the goal is to distill to a student that is considerably smaller than the teacher. Often, this is the case in settings where distillation is used as a compression technique.
% feasible if the teacher model is too complex to deploy in practice, and one desires a student with smaller complexity. 
Yet, this post-hoc method %may still be useful in providing a rough estimate of the worst-case performance that a student can hope to 
% achieve when using a particular teacher, and will 
serves as good baseline to compare with.

% \vspace{-2pt}
\textbf{One-hot validation labels.}\
% \label{sec:one-hot-val}
% \vspace{-2pt}
If Algorithm \ref{algo:dro} used one-hot labels in the validation set instead of the teacher generated labels (as prescribed in \eqref{eq:one-hot-val}),
the form of the student learned remains the same as 
 in Theorem \ref{thm:dro}. However, the coefficients $\bar{\lambda}$ used to make
adjustments to the teacher's predictions enjoy a slightly different guarantee.
% Specifically, 
As shown in Appendix \ref{app:one-hot-vali}, the approximation error bound now has a weaker dependence on the teacher's predictions (and hence is more immune to the teacher's errors),
while the estimation error bound incurs slower convergence with increase in sample size. %We elaborate on the robustness guarantees for this variant in Appendix \ref{app:one-hot-vali}.
